Structural Resolution with Co-inductive Loop Detection

A way to combine co-SLD style loop detection with structural resolution was found and is introduced in this work, to extend structural resolution with co-induction. In particular, we present the operational semantics, called co-inductive structural resolution, of this novel combination and prove its soundness with respect to the greatest complete Herbrand model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{E. Komendantskaya and J. Power (Eds.):\\ Coalgebra, Horn Clause Logic Programming and Types\\
EPTCS 258, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.258.4}{10.4204/EPTCS.258.4}}
\pdfoutput=1

